Evolving Graphical Planner: Contextual Global Planning for Vision-and-Language Navigation

The ability to perform effective planning is crucial for building an instruction-following agent. When navigating through a new environment, an agent is challenged with (1) connecting the natural language instructions with its progressively growing knowledge of the world; and (2) performing long-range planning and decision making in the form of effective exploration and error correction. Current methods are still limited on both fronts despite extensive efforts. In this paper, we introduce the Evolving Graphical Planner (EGP), a model that performs global planning for navigation based on raw sensory input. The model dynamically constructs a graphical representation, generalizes the action space to allow for more flexible decision making, and performs efficient planning on a proxy graph representation. We evaluate our model on a challenging Vision-and-Language Navigation (VLN) task with photorealistic images and achieve superior performance compared to previous navigation architectures. For instance, we achieve a 53% success rate on the test split of the Room-to-Room navigation task through pure imitation learning, outperforming previous navigation architectures by up to 5%.

==> abs.tex <==
The ability to perform effective planning is crucial towards building a general instruction-following agent. When navigating through a new environment, an agent is challenged with handling (1) the understandings between natural language depicting the task and the progressively growing world knowledge; (2) the long-range planning and decision making leading to effective exploration and error correction. Despite with the efforts in language understandings for navigation, existing methods are still limited on the expressive power of decision space and planning ability. In this paper, we propose \textit{Evolving Graphical Planner (EGP)}, a module that performs non-local planning for navigation based on raw sensory input. The module dynamically constructs a graphical representation, generalizes the local action space to allow for more flexible decision making, and performs efficient planning on a proxy representation. We demonstrate our model on a challenging Vision-and-Language Navigation (VLN) task with photorealistic images, and achieve superior performance compared to previous navigation architectures.

%The ability to perform effective planning is crucial towards building a general instruction-following agent. When navigating through a new environment, an agent is challenged with handling (1) the understandings between natural language depicting the whole task and the progressively growing world knowledge; (2) the powerful long-range planning and decision making leading to effective exploration and error correction. When navigating through a new environment, an agent is challenged with handling (1) the understandings between natural language depicting the whole task and the progressively growing world knowledge; (2) the increasing complexity of decision makings involving exploration and error correction. In this paper, we propose \textit{Evolving Graphical Planner (EGP)}, a differentiable module that performs non-local planning for navigation based on raw sensory input. The module dynamically constructs a graphical representation, generalizes the local action space to allow for more flexible decision making, and performs efficient planning on a proxy representation. We demonstrate our model on a challenging Vision-and-Language Navigation (VLN) task with photorealistic images, and achieve superior performance compared to previous navigation architectures.

%In this paper, we address the problem of building autonomous navigation agents guided by instructions. To effectively navigate through a real world unseen environment in one shot, an ideal agent needs to understand instructions, perform long-term planning and build structured understanding among observations and the language to complete the final task. To build towards this, we propose \textit{Evolving Graphical Planner (EGP)}, a differentiable module that performs long-term planning for navigation using raw sensory input. The module: (1) generalizes the local planning space to a global action space represented by a evolving graph, and (2) performs planning on a condensed core, making the unit scalable to larger graphs. In the experiment, we show that the proposed model can achieve state-of-the-art performance on the Vision-and-Language Navigation tasks without bells and whistles.

==> algorithm.tex <==

\begin{wrapfigure}{R}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
    \begin{algorithm}[H]
        \caption{EvolvingGraphExpansion}
        \begin{algorithmic}
          \STATE \textbf{Input:} %Graphical representation $G_{t-1}$; environment \textsc{env}; observation $\vec{o}_{\vec{s}_t}$ of state $\vec{s}_t$, observation set of new actions $\{\vec{o}_{a_k}\}_t$
          \STATE \textbf{Output:} Graphical representation $G_t$
          \STATE$\vec{v_{\vec{s}_t}} \gets \textsc{NN}_s(\vec{o}_{\vec{s}_t})$
          
          \STATE $\mathcal{V}_{new} \gets \{\vec{v_{\vec{s}_t}}\}$
          
          \FOR{$\vec{o} \in \{\vec{o}_{a_k}\}_t$} \STATE {$\vec{v_{a}} \gets \textsc{NN}_a(\vec{o})$}
          
          \STATE {$\mathcal{V}_{new} \gets \mathcal{V}_{new} \cup \{\vec{v_{a}}\}$}
          
          \ENDFOR
          \FOR{$v_{i} \in \mathcal{V}_{new}$} \IF{$v$ is action} \STATE {$\vec{E}[]$} \ELSE \STATE{<text>} \ENDIF 
          \ENDFOR
        \end{algorithmic}
      \end{algorithm}
\end{minipage}
\end{wrapfigure}


==> model_start.tex <==
\section{Model}
In this section, we introduce our \textit{Evolving Graphical Planner (EGP)}, an end-to-end global planner that navigates a agent through a new environment via re-defining the decision space and performing long-term plannings over the graphs. Our proposed model consists of two core components: (1) an evolving graphical representation that generalizes the local action space; (2) a planning core that performs multi-channel information propagation on a proxy representation. Starting from the initial information, the EGP agent gradually expands an internal representation of the explored space (Section \ref{EGP:rep}) and perform planning efficiently over the entire graphs (Section \ref{EGP:core}).


==> preliminaries.tex <==
\section{Background}
%We begin by introducing the problem and the base agent formally. We then describe a core function used in the main model.
\subsection{Problem definition and agent setup}
%\textbf{Instruction-following navigation}
\textbf{Problem definition} We follow the standard instruction-following navigation problem setting \cite{anderson2018vision}. In the task, the agent receives a language instruction $\vec{x}$, an initial state $\vec{s}_0$ and produces a sequence of actions $\vec{\tau} = (a_1, a_2, ..., a_T)$ to navigate through the environment $\textsc{env}$, where $T$ is the episode length.

The agent is trained under the imitation learning setting. Given a set of demonstration data $\mathcal{D} = \{(\vec{x}_i, \vec{\tau}_i^{*}, \textsc{env}_i)\}_{i=1}^{\abs{\mathcal{D}}}$ from the experts, where $\abs{\cdot}$ denotes the size of a set, the agent needs to learn to mimic the demonstration trajectory $\vec{\tau}_i^{*}$ on how to follow the language instruction $\vec{x}_i$. A state sequence $\{\vec{s}_1, \vec{s}_2,..., \vec{s}_T\}$ is produced when the action sequence $\vec{\tau}$ is executed. At each state $\vec{s}_t$, the agent makes an observation $\vec{o}_t$ from the environment. The decision space $\mathcal{A}$ of an agent is normally defined locally according to the state of the agent as $\{a_k\}_{\vec{s}_t}$. For example, $\mathcal{A}$ is a set of navigable locations in \cite{fried2018speaker}.


%Given a natural language instruction $\vec{x}$ and an initial state $\vec{s}_1$ in environment $\textsc{env}$, the agent produces a sequence of actions $\vec{\tau} = (a_1, a_2, ..., a_T)$ to navigate through the environment according to the instruction $\vec{x}$. We build the navigation agent under the imitation learning setting. Given a set of demonstration data $\mathcal{D} = \{(\vec{x}_i, \vec{\tau}_i, \textsc{env}_i)\}_{i=1}^N$ from the experts, the agent needs to learn to mimic the demonstration trajectory $\vec{\tau}_i$ on how to follow the natural language $\vec{x}_i$ to achieve the goal. For every step, the agent receives an observation $\vec{o}_t$ at state $\vec{s}_t$ from the environment after performing an action $a_{t-1} \in \mathcal{A}$. The decision space $\mathcal{A}$ of an agent is normally defined locally according to the state of the agent as $\{a_k\}_{\vec{s}_t}$. For example, $\mathcal{A}$ could be the set of navigable locations at state $\vec{s}_t$ \cite{fried2018speaker}.

%We consider an embodied agent learning to navigate through environments given the corresponding descriptions or instructions. Formally, given a set of demonstration data $\mathcal{D} = \{(\vec{y}_i, \vec{\tau}_i, \textsc{env})_i\}_{i=1}^N$, where $\vec{\tau_i}=(a_1, a_2,...,a_{T_i})$ is the demonstration trajectory paired with the description $\vec{y}_i$, an agent needs to learn to mimic the demonstration $\vec{\tau}_i$ in environment ${\textsc{env}}_i$ to follow the instruction $\vec{y}_i$. At every step when the agent performs an action $a_t$, the corresponding environment provides the corresponding resulting observation $\vec{s}_t$. We assume demonstration data exactly follows the description/instructions and achieves the maximum reward $R(\vec{\tau})$ for corresponding task.

%our goal is to train an agent that can navigate through the environment defined by graph $G$, given the instruction $\vec{y}$. $\vec{\tau}$ is the target trajectory $(\vec{s}_0,\vec{s}_1,...,\vec{s}_T)$. At each step $t$, the agent receives an observation $\vec{v}_t$ from the environment at state (position) $\vec{s}_t$ and performs an action $\vec{a}_t$ to teleport to the next position.

%\textbf{Navigation agent} 

\textbf{Agent setup} We build our base agent upon the sequence-to-sequence model in \cite{ma2019self}. The agent encodes the language instruction $\vec{x}$ through an LSTM \cite{gers1999learning}, into a hidden encoding $\vec{c}=(\vec{c}_1, \vec{c}_1, ..., \vec{c}_M)$ where $M$ is the number of words in $\vec{x}$. Conditioned on $\vec{c}$, the agent uses a decoder to model the distribution over the trajectory as $p(\vec{\tau}|\vec{x}, \textsc{env})$. At every step, the decoder takes in the encoding $\vec{c}$, the observation $\vec{o}_t$ and a maintained hidden memory $\vec{h}_{t-1}$ to produce the action probability distribution $p(a_t|\vec{h}_{t-1}, \vec{o}_t, \vec{c})$. Attention-based models are often used in designing decoders \cite{anderson2018vision, ma2019regretful}. 

%We use the co-grounding module \cite{ma2019self} throughout the paper 

%to produce the route distribution $p(\vec{\tau}|\vec{x})$ given the instruction $\vec{x}$. The model encodes the language instruction through an LSTM \cite{gers1999learning}, into a hidden encoding $\vec{c}=(\vec{c}_1, \vec{c}_1, ..., \vec{c}_M)$ where $M$ is the length of the instruction $\vec{x}$. Based on the language encoding $\vec{c}$, previous decisions $a_{<t}$ and the current observation $\vec{v}_t$, the agent extracts or grounds information through attention-based modules \cite{ma2019self, fried2018speaker} and maintains a hidden state summarizing the history in $\vec{h}_t$. The per-step distribution over actions $p(a_t|\vec{h}_{t-1}, \vec{c})$ could be derived through a dot-product between the hidden encoding $\vec{h}_t$ and the embedding of each actions \cite{fried2018speaker, ma2019self}. Being constrained to making local decisions, the agent has shown issues on correcting  mistakes, effectively exploring the new environment or acquiring long-term planning ability \cite{fang2019scene, ma2019regretful, ke2019tactical}.

%(Talk about constraints, also ask some questions)

%Being constrained to making local decisions, the agent has shown issues on correcting  mistakes, effectively exploring the new environment or acquiring long-term planning ability \cite{fang2019scene, ma2019regretful, ke2019tactical}. 

\subsection{Graph Neural Networks}
\label{pre:GNN}
Graph Neural Network (GNN) is standard model used for propagating information between a set of elements. We summarize the GNN as a function in this section. Denote the initial graph as $\mathcal{G}=(\mathcal{V}_0, \mathcal{E}_0, \vec{M})$, where $\mathcal{V}_0$ and $\mathcal{E}_0$ represent the set of node vectors $\{\vec{v}_0^i\}, \vec{v}_0^i\in \mathbb{R}^{d_{\text{in}}}$ and the set of edge vectors $\{\vec{e}_0^{ij}\}$ respectively, and $\vec{M} \in \mathbb{R}^{\abs{\mathcal{V}}\times\abs{\mathcal{V}}\times\abs{\mathcal{F}}}$ denotes the message type matrix with non-negative real-value weights ($\mathcal{F}$ is the set of message types). The $\textsc{GNN}$ function takes in the graph and a context vector $\vec{r}$ and generates the refined node vectors $\mathcal{V}_K$ after $K$ steps of message passings through $\textsc{GNN}(\mathcal{G}, \vec{r}; K, d_{\mathcal{G}})$, where $d_{\mathcal{G}}$ is the vector dimension in the propagation model.

\textbf{Input model} Along with the initial vectors for nodes and edges, the model considers a context vector $\vec{r}$ representing a shared additional information across nodes. The input model maps the context vector with node and edge vectors respectively into two fixed-size embedding as follows:
\begin{equation}
    \vec{v}_1^i=f_{\text{in}}(\vec{v}_0^i, \vec{r}); 
    \vec{e}_1^{ij}=f_{\text{in}}(\vec{e}_0^{ij}, \vec{r}); \vec{v}_1^i, \vec{e}_1^{ij} \in \mathbb{R}^{d_{\mathcal{G}}}
\end{equation}
where $f_{\text{in}}$ is a neural network, and the generated embedding vectors are used for message communications among graph nodes in the propagation model.

\textbf{Propagation model} The propagation model, taking in the mapped embedding vectors $\{\vec{v}^i_1\}$, consecutively generates a sequence of node embedding vectors $(\vec{v}_2^i, \vec{v}_3^i, ..., \vec{v}_{K+1}^i), k\in \{1,...,K+1\}$ for each node. At step $k$, the propagation operation updates every node through computing and aggregating information from the neighborhood nodes. The process is executed in the order:
\begin{eqnarray}
    \vec{e}_k^{ij} &=& \sum_n \vec{M}_{i,j,n}\cdot f_{n}\Big(\vec{v}_k^i, \vec{v}_k^j, \vec{e}_1^{ij}\Big) \in \mathbb{R}^{d_{\mathcal{G}}};
    \\
    \vec{v}_{k+1}^i &=& g\Big(\sum_{j\in \mathcal{N}_i}\vec{e}_k^{ij}, \vec{v}_{k}^i\Big) 
    \in \mathbb{R}^{d_{\mathcal{G}}}
\end{eqnarray}
where $f_n(\cdot,\cdot,\cdot): \mathbb{R}^{3d} \rightarrow \mathbb{R}^d$ is the message function. Function $g(\cdot): \mathbb{R}^{2d} \rightarrow \mathbb{R}^d$ is the aggregator function that collects messages back to node vectors. $\mathcal{N}_i$ represents the neighbours of node $i$ in the graph. The whole propagation process is repeated for $K$ times. The the refined node vector set $\{\vec{v}_{K+1}^i\}$, containing global information from the whole graph is mapped through a matrix $W_{\text{out}}$ to recover the input node dimension $d_{\text{in}}$.


==> pull_fig.tex <==

\begin{wrapfigure}{R}{0.35\textwidth}
\begin{center}
\includegraphics[width=0.35\textwidth]{figs/pull_fig.pdf}
  \caption{The Evolving Graphical Planner generates non-local actions for agent to navigate through the unseen environments. \olga{this figure isn't doing much for me, might be better to remove and expand the text}}
\label{fig:main_fig}
\end{center}
\end{wrapfigure}


==> vln_forcing_table.tex <==

\begin{table}[h!]
\centering
{\small
\begin{tabular}{c c c c c c c c}
  \toprule
    Models & PL $\downarrow$ & NE $\downarrow$ & SR $\uparrow$ & SPL $\uparrow$ & OSR $\uparrow$
    \\
    \hline
    EGP - with shortest path & 14.68 & 5.65 & 0.46 & 0.36 & 0.57
    \\
    EGP - with graph-GT & 13.68 & 5.34 & 0.52 & 0.41 & 0.65
    \\ \bottomrule
    \end{tabular}
    }
  \caption{Comparison between two supervision methods for student forcing. The graph-GT method provides supervision with less noisy and mismatched actions, leading to higher performance.}
  \label{tbl:forcing}
  \vspace{-3mm}
\end{table}
